Cafe-Mpc: A Cascaded-Fidelity Model Predictive Control Framework with Tuning-Free Whole-Body Control

This work introduces an optimization-based locomotion control framework for on-the-fly synthesis of complex dynamic maneuvers. At the core of the proposed framework is a cascaded-fidelity model predictive controller (Cafe-Mpc). Cafe-Mpc strategically relaxes the planning problem along the prediction horizon (i.e., with descending model fidelity, increasingly coarse time steps, and relaxed constraints) for computational and performance gains. This problem is numerically solved with an efficient customized multiple-shooting iLQR (MS-iLQR) solver that is tailored for hybrid systems. The action-value function from Cafe-Mpc is then used as the basis for a new value-function-based whole-body control (VWBC) technique that avoids additional tuning for the WBC. In this respect, the proposed framework unifies whole-body MPC and more conventional whole-body quadratic programming (QP), which have been treated as separate components in previous works. We study the effects of the cascaded relaxations in Cafe-Mpc on the tracking performance and required computation time. We also show that the Cafe-Mpc, if configured appropriately, advances the performance of whole-body MPC without necessarily increasing computational cost. Further, we show the superior performance of the proposed VWBC over the Riccati feedback controller in terms of constraint handling. The proposed framework enables accomplishing for the first time gymnastic-style running barrel rolls on the MIT Mini Cheetah. Video: https://youtu.be/YiNqrgj9mb8.

==> MS_01/WBMPC.tex <==

\subsubsection{Comparison to Whole-Body MPC} In a final investigation, we compare state-of-the-art whole-body MPC with the proposed {\sc Cafe-Mpc} regarding their capability to achieve the Fosbury Flop. Note that the whole-body MPC is equivalent to {\sc Cafe-Mpc} with zero-length SRB plan (i.e., $T_s=0$). The whole-body MPC is executed at 50 Hz with run-time constraints (18 ms) on solving the underlying optimization problems. The prediction horizon $T_w$ is varied between 0.3 s and 0.6 s, with an increment of 0.1 s. For each horizon we conduct twenty almost-identical tests in simulation, which are only slightly different from each other due to the sensor noise realizations and slight MPC solve-time variations. With $T_w <= 0.4$ s, zero successes are achieved, and with $T_w = 0.5$ s, one success is achieved out of twenty tests. All failures happen because of unstable landings. Note that the air phase of the barrel roll is 0.36 s. The unstable landing is likely because the MPC synthesized take-off does not cover sufficiently long after landing. Extending $T_w$ to 0.6 s helps improve the success rate of whole-body MPC to $50.5\%$ in simulation, which was the best-case scenario for whole-body MPC. Note that the \cmpc shows $100\%$ success in the simulation tests. Those failed simulation tests for whole-body MPC likely result from insufficient computation speed, since the average number of solver iterations is limited to 1.5 due to the run-time constraints, whereas this number is 4 for {\sc Cafe-Mpc}. To test this argument, we run the simulation at half speed, and allow the whole-body MPC solver to run a maximum 4 iterations, resulting 100$\%$ success rate. Elongating $T_w$ to 0.8 s further reduces the average solver iterations, dropping the success rate to $10\%$ when the simulation is run at a real-time rate. In a nutshell, for whole-body MPC to synthesize the running barrel roll, the planning horizon needs to be sufficiently long, which on the other hand, significantly increases the computational difficulty, thus preventing robust success even in an idealized simulation. Speeding up computation time for whole-body MPC is a vibrant research area \cite{mastalli2023inverse, jallet2023proxddp}. The real-time iteration scheme \cite{diehl2005real}\cite{grandia2023perceptive} also shows the promise of solving for only one iteration. We anticipate that whole-body MPC has the potential to execute a barrel roll on hardware in the foreseeable future. Nonetheless, it is worth noting that our approach offers a straightforward yet powerful means of integrating whole-body planning into MPC in a way that allows for extending the horizon with low additional computational overhead.
